LogicENN: A Neural Based Knowledge Graphs Embedding Model with Logical Rules

Knowledge graph embedding models have gained significant attention in AI research. Recent works have shown that the inclusion of background knowledge, such as logical rules, can improve the performance of embeddings in downstream machine learning tasks. However, so far, most existing models do not allow the inclusion of rules. We address the challenge of including rules and present a new neural based embedding model (LogicENN). We prove that LogicENN can learn every ground truth of encoded rules in a knowledge graph. To the best of our knowledge, this has not been proved so far for the neural based family of embedding models. Moreover, we derive formulae for the inclusion of various rules, including (anti-)symmetric, inverse, irreflexive and transitive, implication, composition, equivalence and negation. Our formulation allows to avoid grounding for implication and equivalence relations. Our experiments show that LogicENN outperforms the state-of-the-art models in link prediction.

==> oldstuff.tex <==


\section{OLD STUFF}
 


Generally, knowledge graph embedding models have the following main components in common:
\begin{itemize}
    \item Parameters of an embedding model ($\Theta$) which includes embedding vectors and parameters of the score function 
    
    \item An score function is denoted by $f^r(h,t)$ or $f^r_{h,t}$ which gets the embedding vectors of a triple and returns the degree of its correctness.
    Different embedding models propose different score functions. 
    
    \item A loss function, which is denoted by $\mathcal{L}$, is optimized over embedding vectors and score function parameters. Two widely used loss function in KGE literature are margin ranking loss and negative likelihood loss:
    \begin{itemize}
        \item Margin ranking loss: 
        $$\mathcal{L} = \sum_{(h,r,t) \in \mathcal{S}, (h^{'},r,t^{'}) \in \mathcal{S^{'}} } [\lambda + f^r(h,t) - f^r(h^{'},t^{'})]_+ $$
        
        where $\lambda$ is margin, $(u^{'},r,v^{'})$ is a corrupted triple acting as a negative example and $[x
        ]_+=\max(0,x)$.
        
        \item Negative log-likelihood loss: 
        $$\mathcal{L} = \sum_{(h,r,t)\in \mathcal{S} } log(1+exp(-y_{h,t}^r\, f^r_{h,t}))$$
        \hamed{what is $-y_{h,t}^r$?}
        
    \end{itemize}
    
    \item Some KGE methods use constraints or regularization terms. The former is used to restrict the solution space of the optimization problem. The later is used to provide a trade of between some user determined criteria and the loss. 
\end{itemize}

 

 
Regarding the first question, TransE is not capable of encoding some rules
including reflexive ~\cite{TransH} as well as symmetric and transitive ~\cite{LogicTransX}. 
Recently, ~\cite{SimplE} proves that not only TransE, but also many of its variants such as FTransE ~\cite{FtransE}, STransE ~\cite{StransE}, TransH
[41], and TransR ~\cite{TransR} are not fully expressive, meaning that some rules cannot be encoded by them. \hamed{we mix up many patterns.
It is better that we categorize models based on patterns or the other way to make the text readily understandable}

DistMult ~\cite{Distmult} cannot capture antisymmetric relations while ComplEx ~\cite{ComplEx} can encode symmetric and antisymmetric relations due to use of complex conjugate of embeddings. \hamed{How?}
Authors in \cite{ComplexJourn} indicate that Canonical Polyadic (CP) \cite{CPdecomp} decomposition cannot encode both symmetric and antisymmetric relations. ~\cite{ProofPaper} comprehensively investigates the expressiveness of different bilinear models. 
It investigates the subsumption relations between the embedding models. 
According to ~\cite{ProofPaper}, an embedding model is universal if it can express any ranking tensors.
Theoretical proofs ~\cite{ProofPaper} show that ComplEx ~\cite{ComplEx}, HolE ~\cite{HolE} and RESCAL ~\cite{RESCAL} are universal under specific constraints.
SimplE is one the recent embedding model which is proven to be fully expressive. Conditions for encoding symmetric, anti-symmetric and inverse patterns are mentioned in ~\cite{SimplE}. 
 


 

Regarding the second question, there is not a unique solution to encode different logical rules and relation patterns in an embedding model. 
In another word, different embedding models favor different ways for suitable rule injection.
~\cite{rocktaschel2015injecting} first applies pre-factorization inference with logical rules to include new inferred triples in training data. 
This process is iterated until no new facts are inferred. 
Then, it treats both ground atoms and logical backgrounds as logical formulae and computes the marginal probability of the formulae included in the training set. The loss function is created on the top of the marginal probabilities. 
KALE ~\cite{guo2016jointly} uses margin ranking loss over logical formulae and triple facts. Therefore, it jointly learns from triples and formulae. 
In order not be relied on propositionalization for implication rule, ~\cite{demeester2016lifted} proposes lifted rule injection. Methods which consider relation path, which is closely connected to the logical rules, are also well-studied in the literature and can be found in ~\cite{RelationPathneelakantan2015compositional}, ~\cite{RelationPathlin2015modeling}. ~\cite{Relationpathguu2015traversing}. 


 

 
Regarding the second question, there is not a unique solution to encode different logical rules and relation patterns in an embedding model. 
In another word, different embedding models favor different ways for suitable rule injection.
~\cite{rocktaschel2015injecting} first applies pre-factorization inference with logical rules to include new inferred triples in training data. 
This process is iterated until no new facts are inferred. 
Then, it treats both ground atoms and logical backgrounds as logical formulae and computes the marginal probability of the formulae included in the training set. The loss function is created on the top of the marginal probabilities. 
KALE ~\cite{guo2016jointly} uses margin ranking loss over logical formulae and triple facts. Therefore, it jointly learns from triples and formulae. 
In order not be relied on propositionalization for implication rule, ~\cite{demeester2016lifted} proposes lifted rule injection. Methods which consider relation path, which is closely connected to the logical rules, are also well-studied in the literature and can be found in ~\cite{RelationPathneelakantan2015compositional}, ~\cite{RelationPathlin2015modeling}. ~\cite{Relationpathguu2015traversing}. 
 
RUGE ~\cite{guo2018RUGE} presents a general model independent framework to inject Horn clause soft rules with confidence scores into an embedding model. The rules are encoded as constraints for an optimization problem. 
%It finds soft labels for unlabeled triples iteratively to update embedding vectors and it is conjectured that this approach could better transfer background knowledge from rules to embedding vectors. 
In contrast to RGUE, ~\cite{SimpConstding2018improving} follows model dependent approach for injection of rules. It encodes non-negativity and entailment as constraints for ComplEx model. It is shown in ~\cite{SimpConstding2018improving} that the model dependent approach ~\cite{SimpConstding2018improving} outperforms model independent approach ~\cite{guo2018RUGE} on FB15K dataset. 
 


 

\subsubsection{Neural network based embedding model}
Table \ref{tbl:NNEs} specifies the score functions of different neural based embedding models. 

\textbf{E-MLP} \cite{socher2013reasoning} which is standard Multi Layer Perceptron (MLP) for KGE. E-MLP uses one neural network per each relations in the KG which has high space complexity. 

\textbf{ER-MLP} \cite{ER-MLPdong2014knowledge} In contrast to E-MLP which uses one neural network per each relation, ER-MLP shares its weights between all entities and relations. The relation embedding is placed as input of the network. 

\textbf{NTN} \cite{socher2013reasoning} employs 3-way tensor in the hidden layer to better capture interactions between features of two entities. The score function of NTN is as follows:
\begin{align}
    f^r_{u,v} = \boldsymbol{w}_{1r}^T \tanh(\boldsymbol{u}^T \boldsymbol{W}_{0htr}\boldsymbol{v} + W_{0hr} \boldsymbol{u} + W_{0tr} \boldsymbol{v} + b_r)
\end{align}

where $\boldsymbol{W}_{0htr} \in \mathbb{R}^{d\times d\times L}, b_r \in \mathbb{R}^L$ are the 3-way relation specific tensor and bias of hidden layer respectively. 

\textbf{ConvE} ~\cite{ConvEdettmers2018convolutional} is a multi-layer convolutional network for link prediction. The score function of ConvE is as follows:
\begin{align}
    f^r_{u,v} = g(\text{Vec}(g([\Bar{\boldsymbol{u}};\Bar{\boldsymbol{r}}]*\omega))W)\boldsymbol{v}
\end{align}
where $\omega$ is filter and $W$ is a linear transformation matrix. $g$ is an activation function. 
\hamed{What does upper line means in $\Bar{\boldsymbol{u}}$? 
Also "Vec"?}

\textbf{ConvKB} ~\cite{ConvKBnguyen2017novel} is a multi-layer convolutional network for link prediction with the following score function:

\begin{align}
    f^r_{u,v} = \text{Concat}(g([\Bar{\boldsymbol{u}};\Bar{\boldsymbol{r}},\Bar{\boldsymbol{v}}]*\omega))W
\end{align}
\hamed{What does Concat do on the output of function "g"?}

\textbf{Other neural based embedding models}

\textbf{SENN} ~\cite{SENNguan2018shared} defines three multi-layer neural networks with Relu activation function for head, relation and tail prediction. Then, it integrates them into one loss function to train the model.

\textbf{TBNN} ~\cite{TBNNhan2018triple} is a triple branch neural network in which parallel branched layers are defined on the top of an interaction layer where each embedding of any element of a KG is specified by its multi restriction. The loss function is defined based on the score of three elements of each triple.

\textbf{ProjE} ~\cite{projeshi2017} is a two layer neural network. The first layer is a combination layer which works on tail and relation and the second layer is a projection layer which projects the obtained vector from the last layer to the candidate-entity matrix. The candidate-entity matrix is a subset of entity matrix where entities can be sampled in different ways. 


\subsubsection{KGE with logical rules}

\textbf{RUGE}
provides a general framework to iteratively inject logical rules in KGE. Given a set of soft logical rules $\mathcal{R} = \{(l_p, \lambda_p)\}$ where $l_p$ is a FOL rule \hamed{need to be defined} and $l_p$ is its confidence value, rules are represented as mathematical  constraints to obtain soft labels for unlabeled triples. Then, an optimization problem is solved to update embedding vectors based on hard and soft labeled triples. The framework is used to train ComplEx model as case study. 

\textbf{ComplEx-NNE+AER} ~\cite{SimpConstding2018improving}, which is a model dependent approach, derives formula for entailment rule to avoid grounding in ComplEx. The model outperforms RUGE on FB15K in the terms of Meanrank and Hit@k.
 

 
\subsection{Analyzing related works and motivation}
\hamed{the materials here are here and there mentioned earlier.
It is better to change the name of this section to something like
"Summary of the literature review and open problems".
We should rewrite it again.
}
Encoding logical rules as mathematical constraints has recently attracted attention. RUGE provides a general framework for rule injection which is model independent, i.e.\ it can be applied to any embedding models. Deriving mathematical constraints for logical rules by considering characteristic of embedding model (model dependent approach) has some advantages. For example, Both RUGE and ComplEx-NNE+AER use ComplEx as based embedding model for rule injection. But ComplEx-NNE+AER derives mathematical constraints for implication rule based on ComplEx which doesn't need any grounding. This cannot be done in RUGE framework. 
Therefore, developing a flexible embedding model which is capable of encoding different rules and deriving model dependent mathematical constraints is of interest. 
We found that neural networks are very flexible for encoding rules. However, flexibility depends on the design of a neural network. Most of existing neural networks consider relation as input or hidden layer weight. This non-linearity over relations reduce the flexibility of the models to include logical rules especially avoid grounding for some specific rules.
 

 
\begin{table}
\centering
\begin{tabular}{ll}
\toprule %\hline
Notation  & Meaning\\
\midrule %\hline
$(h,r,t)$  & {Triple Fact}\\
$h,r,t$  & head, relation and tail respectively\\

$\vec{h}, \vec{r}, \vec{t}$  & Embedding vectors of $h, r, t$\\



$n_e$  & {Number of entities}\\

$n_r$  & {Number of relations}\\

$w^l$  & {l-th hidden layer weights}\\

$\beta^r$  & {Input weights of the r-th output node}\\

$\phi_{uv}^l$  & {l-th hidden layer mapping}\\

$\phi_{uv}$  & {Mapping of the last hidden layer}\\

$n_l$  & {Number of nodes in the l-th hidden layer}\\

$\vec{x} = [\vec{h};\vec{t}]$  & {Concatenation of head and tail vectors}\\

$\Omega$ & {input space}\\

$\mathcal{A}$ & {Sigma algebra}\\

$\mu$ & measure\\

\bottomrule %\hline
\end{tabular}
\caption{Variable specification}
\label{tbl:specifications}
\end{table}
 


 


\hamed{In table-\ref{tbl:specifications} We should use consistent notation, better to use $h,t$ instead of $u,v$}

\newpage
\begin{table}
\centering
\begin{tabular}{lll}
\toprule %\hline
Method  & Score Function & Loss \\
\midrule %\hline
TransE  & 0.1s \\
Distmult  & 0.1s \\
TransH  & 0.1s \\
TransD  & 0.1s \\
TransR  & 0.1s \\
ComplEx  & 0.1s \\
ANALOGY & 0.1s \\
HolE & 0.1s \\
RESCAL & 0.1s \\
Unstructured & 0.1s \\
SME & 0.1s \\
LFM & 0.1s \\
E-MLP  & 0.1s \\
ER-MLP & 0.2s \\
NTN    & 0.1s \\
ConvE  & 0.1s \\
ConvKB & 0.2s \\
Neural LP & 0.2s \\
IRNs & 0.2s (20 negative samples) \\
DKRL & f \\
\bottomrule %\hline
\end{tabular}
\caption{Number of parameters of different models and the proposed+
LogicNN.}
\label{tbl:parameters}
\end{table}
\hamed{do wee need this table \ref{tbl:parameters}?}

 


 

\paragraph{Reduced Math constraints}
Reduced Math constraints for 
equivalence is: $ \overrightarrow{1}^T(\vec{w}^{r_1}-\vec{w}^{r_2}) = \xi_{r_1,r_2}$ \\
For Implication is:
$ \vec{w}^{r_1}-\vec{w}^{r_2} \leq \overrightarrow{0}$
 


 
\subsection{Dataset}
We evaluate our proposed models on two datasets: FB15k and WN18 \cite{bordes2013translating}, where there exist various logical rules among relations. The statistics of the dataset are listed in Table.

\begin{table}[]
    \centering
    \begin{tabular}{c|ccccc}
    \toprule
         Dataset&\#Rel&\#Ent&\#Train&\#Valid&\#Test \\
    \midrule
         FB15k&1,345&14,951&483,142&50,000&59,071\\
         WN18&18&40,943&141,442&5,000&5,000\\
    \bottomrule
    \end{tabular}
    \caption{Statics of datasets}
    \label{tab:Statics of datasets}
\end{table}

We further employ AMIE+~\cite{galarraga2015AMIE+} to extract Horn clause rules from the training sets of these two dataset. For efficient extraction, we set the length of rules no longer than 2. And the confidence levels of rules are supposed to be no less than 0.8. Using this setting, we extract 454 and 14 Horn clause rules respectively from FB15k and WN18. For formulating different rules, we categorize rules mined from datasets according to the definitions in Table \ref{tbl:LogicalConstraints}. Then we instantiate these rules with concrete triples in training sets. For instance, given a Horn clause rule $\forall x,y: (x, \text{isMarriedTo}, y)\Leftrightarrow(y, \text{isMarriedTo}, x)$ and an observed triple (Barack Obama, isMarriedTo, Michelle Obama) in the training set, we can generate a resultant grounding: $(\text{Barack Obama}, \text{isMarriedTo}, \text{Michelle Obama})\Leftrightarrow(\text{Mchelle Obama}, \text{isMarriedTo}, \text{Barack Obama})$. Similar to RUGE, we only take as valid groundings those where premise triple are observed in the training set, while conclusion triples are not, to maximize the utility for knowledge acquisition and inference. The numbers of different types of rules and groundings on FB15k and WN18 are listed in Table~\ref{tbl:RuleNumbers}
 

 
\begin{table}[]
    \centering
    \footnotesize
    \begin{tabular}{ccccccc}
    \toprule
    %&\multicolumn{6}{c}{FB15k}\cr
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}
    &MR&Hits@10&MRR\cr
    \midrule
    LogicENN$_R$&320&40.2&18.1\cr
    LogicENN$_R$+Inverse$^\star$&\textbf{187}&\textbf{62.1}&\textbf{37.7}\cr
    LogicENN$_R$+Implication&321&40.5&18.2\cr
    LogicENN$_R$+Symmetry&299&42.2&18.5\cr
    LogicENN$_R$+Equivalency&302&41.7&19.0\cr
    LogicENN$_R$+Composition&303&41.0&18.1\cr
    \midrule
    LogicENN$_S$&430&36.6&15.2\cr
    LogicENN$_S$+Inverse$^\star$&\textbf{180}&\textbf{59.3}&\textbf{35.2}\cr
    LogicENN$_S$+Implication&421&37.1&16.4\cr
    LogicENN$_S$+Symmetry&387&37.9&17.2\cr
    LogicENN$_S$+Equivalency&330&38.4&17.7\cr
    LogicENN$_S$+Compositiony&391&37.1&16.0\cr
    \bottomrule
    \end{tabular}
    \caption{
    Link prediction results with different activation functions and rules on FB15k.
    $\star$ indicates that the proposed model outperforms all baseline models}
    \label{tbl:ResultsWithRules}
\end{table}

 



There, vectors of are denoted by bold non-capital letters (e.g.\ $\vec{h}$ or $\vec{0},\vec{1}$ as vectors of zeros and ones respectively), matrices by bold capital letters and tensors by underlined bold capital letters.
$\mat{W}^{(.)}$ are weight matrices which have no dependency on $h$, $r$ or $t$, while $\mat{W}^{(.)}_{r}$ ($\ten{W}_{r}$) means that the weight matrix (tensor) is associated to relation $r$.
Moreover, $\Bar{\vec{h}}, \Bar{\vec{r}}$ and $\Bar{\vec{t}}$ are 2D-reshape of $h$, $r$ and $t$ respectively.




\paragraph{???????????}
As another example, assume that we would like to encode an implication for relations ``bornInCountry'' and ``hasNationality''.
We can represent it as a rule like 
$\forall \var{x},\var{y}: (\var{x},\text{bornInCountry},\var{y})\Rightarrow (\var{x},\text{hasNationality},\var{y})$.

==> tab_used_rules.tex <==
\begin{table}[]
    \centering
    \footnotesize
    \begin{tabular}{lcccc}
    \toprule
    &\multicolumn{2}{c}{FB15k}&\multicolumn{2}{c}{WN18}\cr
    \cmidrule(lr){2-3}\cmidrule(lr){4-5}
    &Rule&Grounding&Rule&Grounding\cr
    \midrule
    Inverse&292&67757&14&109206\cr
    Implication&30&3259&NA&NA\cr
    Symmetry&24&7745&NA&NA\cr
    Equivalency&68&8771&NA&NA\cr
    Composition&40&7951&NA&NA\cr
    \midrule
    In total&454&95483&14&109206\cr
    \bottomrule
    \end{tabular}
    \caption{Numbers of different rules and groundings in FB15k and WN18 (NA: Relation Not Available).}
    \label{tbl:UsedRules}
\end{table}
